Towards a GML-Enabled Knowledge Graph Platform

This vision paper proposes KGNet, an on-demand graph machine learning (GML) as a service on top of RDF engines to support GML-enabled SPARQL queries. KGNet automates the training of GML models on a KG by identifying a task-specific subgraph. This helps reduce the task-irrelevant KG structure and properties for better scalability and accuracy. While training a GML model on KG, KGNet collects metadata of trained models in the form of an RDF graph called KGMeta, which is interlinked with the relevant subgraphs in KG. Finally, all trained models are accessible via a SPARQL-like query. We call it a GML-enabled query and refer to it as SPARQLML. KGNet supports SPARQLML on top of existing RDF engines as an interface for querying and inferencing over KGs using GML models. The development of KGNet poses research opportunities in several areas, including meta-sampling for identifying task-specific subgraphs, GML pipeline automation with computational constraints, such as limited time and memory budget, and SPARQLML query optimization. KGNet supports different GML tasks, such as node classification, link prediction, and semantic entity matching. We evaluated KGNet using two real KGs of different application domains. Compared to training on the entire KG, KGNet significantly reduced training time and memory usage while maintaining comparable or improved accuracy. The KGNet source-code is available for further study

==> sections/introduction-Essam1.tex <==
\section{Introduction}
\label{sec:intro} 

Knowledge graphs (KGs) are constructed based on semantics captured from heterogeneous datasets using various Artificial Intelligence (AI) techniques, such as representation learning and classification models~\cite{Knowledge_Graphs_Hogan}. Graph machine learning (GML) techniques, such as graph representation learning and graph neural networks (GNNs), are widely used in several data science tasks on KGs of diverse application domains, such as categorizing social behaviour in videos~\cite{SunJL20}, drug-drug interaction~\cite{KGNN} and fraud detection~\cite{CARE-GNN}. In these applications, several problems are formalized as GML models for node classification, link prediction, or semantic entity matching tasks. These GML models are trained using different GML methods. We refer to this type of discovery and exploration as \emph{GML-enabled queries} ($Q^{GML}$), in which a trained GML model is applied to a specific set of sub-graphs.

RDF engines, which are widely used to store KGs~\cite{SaleemKG2022}, and the SPARQL query language do not support GML-enabled queries. Thus, data scientists are fully responsible for developing ML pipelines to train GML models and apply them to KGs in isolation from RDF engines. For KGs, enabling GML-based queries is a more challenging task due to the dynamic schema of KGs and a wide range of KG embedding (KGE) and GNN methods that could be used in several applications for heterogeneous graphs~\cite{GNN_Survey_2021, KG-Embedding-Survey}. It is impractical for average users to have this responsibility.

\begin{figure}[t]
% \ncp\ncp\ncp\ncp
\centering
  \includegraphics[width=\columnwidth]{figures/Paper_Venue_KG_DBLP.pdf}  
  \ncp\ncp\ncp
  \caption{A KG with nodes/edges in red, which could be predicted by classification and link prediction models on the fly.\shorten}
  \label{fig:Paper_Venue_KG}
  % \ncp\ncp\ncp\ncp
\end{figure}

\begin{figure}[t]
\lstdefinestyle{myStyle}{basicstyle=\small\ttfamily, language=SPARQL }
\begin{lstlisting}[style=myStyle,captionpos=b,showspaces=false,frame=singlem,numbers=left,xleftmargin=0.5cm,morekeywords={kgnet, getNodeClass,dblp},escapechar=\%]
prefix dblp: <https://www.dblp.org/>
prefix kgnet: <https://www.kgnet.com/>
select ?title ?venue
where { 
?paper a dblp:Publication.
?paper dblp:title ?title.
?paper %\textbf{?NodeClassifier}% ?venue.
?NodeClassifier a %\textcolor{purple}{ \textbf{kgnet:NodeClassifier}}%.
?NodeClassifier kgnet:TargetNode dblp:Publication.
?NodeClassifier kgnet:NodeLabel dblp:venue.}
\end{lstlisting}
% \ncp\ncp\ncp\ncp
\caption{$Q^{pv}_{GML}$: a SPARQL GML-enabled query using a node classification model to predict a paper's venue on the fly.}
\label{fig:paperVenueSPARQL}
% \ncp\ncp\ncp\ncp\ncp
\end{figure}

The KG illustrated in Figure~\ref{fig:Paper_Venue_KG} contains information about published papers in DBLP~\cite{KG_DBLP}. Traditional SPARQL query language cannot apply GML models on top of a KG, i.e., predict a graph node’s class or a missing affiliation link for an author. For example, the venue node in Figure~\ref{fig:Paper_Venue_KG} is a virtual node that could be predicted using a node classification model. It will be interesting to query this KG to \emph{get the paper-venue node using a GML node classification model via a SPARQL query.} There is a need for seamless integration of GML Models into RDF engines. Thus, users should be able to easily express their GML-enabled queries by following the SPARQL logic of pattern matching, i.e., avoid the explicit use of user-defined functions (UDF).\shorten

We envision a system to automatically train GML models and maintain metadata of trained models as an RDF graph (\emph{Meta-GML KG}). The Meta-GML KG is interlinked with the target-node type in the data KG to enable querying both graphs using SPARQL, as illustrated in $Q^{GML}_V$ in Figure~\ref{fig:paperVenueSPARQL}. This query predicts a venue for each paper using a model of type \emph{kgnet:NodeClassifier}. The GML-enabled triple patterns in lines 8-10 will dereference all \emph{kgnet:NodeClassifier} models that are associated with DBLP nodes of type \emph{dblp:Publication} and predict a class of type \emph{dblp:venue}. We refer to \emph{?NodeClassifier} in the triple pattern \RDFTYPE{?paper}{?NodeClassifier}{?venue} as a \emph{user-defined predicate}. 
Extending RDF engines to support user-defined predicates raises research challenges, such as \myNum{i} automatic training of GML models for different tasks, \myNum{ii} optimizing $Q^{GML}$ for GML model selection based on accuracy and inference time, and \myNum{iii} interacting efficiently with the selected model during the query execution time. 

There is a growing adoption of integrating GML with existing graph databases, such as Neo4j~\cite{Neo4j_semantic_similarity} or Stardog~\cite{Stardog-ML}. However, the above challenges are not addressed by existing graph databases. For example, Neo4j supports some machine learning primitive methods, e.g., PageRank, and shortest-path using the \emph{Cypher} language. Even more, Neo4j Graph Data Science v2.2~\cite{Neo4j_DS} supports limited graph embedding methods in a beta version, such as FastRP, Node2Vec, and Graph Sage. However, a user has to train the models separately as an initial step. Addressing these challenges will bring graph machine learning to data stored in RDF engines instead of getting data to machine learning pipelines. This will encourage the development of KG data science libraries powered by the expressiveness of SPARQL for better analysis and insight discovery based on KG structure and semantics. These libraries will empower data scientists with a full breadth of KG machine learning services on top of KGs stored RDF engines.    


% In this vision paper, we propose {\sysName}, a GML-enabled KG engine. {\sysName} extends existing RDF engines with a \textit{GML-enabled query operators} that interacts with an embedding store and GML services.  Our GML as a service supports a repository of GNN methods and  KGE methods.
% {\sysName} also includes a GML-enabled query engine to transparently maintain the GML graph from the metadata of trained models and optimize the execution of GML-enabled SPARQL queries. Users can query and update trained model metadata using SPARQL queries. The GML-enabled query engine addresses several research challenges,  such as 1) deciding the GML method that best fits the user query i.e. the task required resources for a given KG such as the task type (GML operator), the available compute resources, and the user budget (preferences). 2) estimating the cost of executing GML operators. And finally, 3) a KG data sampler that samples a smaller sub-graph related to the task to avoid full graph training for higher performance and scalability. A basic node similarity search implementation of {\sysName} is demonstrated in \cite{KGNET_DEMO}. {\sysName} is a proof-of-concept system that poses several research opportunities for developing a scalable GML-enabled KG engine. 


This vision paper proposes {\sysName}, a GML-enabled KG engine. {\sysName} extends existing RDF engines with two main components GML-enabled query manager and GML as a Service (GMLaaS). Our query manager transparently maintains the Meta-GML KG from the metadata of trained models, optimizes the GML model selection, and finally rewrites the $Q^{GML}$ query as a SPARQL query. The rewritten SPARQL query interacts with our GMLaaS via HTTP calls to get the prediction from a particular pre-trained model. GMLaaS supports a repository of GNN and KGE methods and automates the training pipelines to model a specific task based on our task-oriented sampling. The automated pipeline can work to meet a user's budget for training the task within a certain time or memory budget. Our task-based sampling allows {\sysName} to avoid training using the full graph for higher performance and scalability.\shorten

In summary, the contributions of this paper are:
\begin{itemize}
\item The first GML-enabled KG platform as an extension of existing RDF stores~\footnote{
 The {\sysName} repository can be accessed at \url{https://gitfront.io/r/CODS/qVzfHvorVyBt/KGNET/}. We will publish the code of {\sysName} and datasets as an open source upon acceptance.}. 
 \item GML as a service to provide automatic training of GML models based on a given memory or time budget.
\item GML-enabled query manager to optimize the GML model selection, i.e., opt for the near-optimal model based on  constraints on accuracy and inference time. 
\item A comprehensive evaluation using three GML tasks on real KGs using different GML methods. Using {\sysName} KG task-based sampling, we achieved 62\% memory reduction and 35\% faster training while achieving similar or better accuracy w.r.t training using the full KG.
\end{itemize}


The remainder of this paper is organized as follows. 
Section ~\ref{sec:GML-pipeline-for-KG} provides a background about existing graph machine learning pipelines. 
Section~\ref{sec:ChallengesOfAutomatingCognitiveQuery} outlines the main research challenges of developing  a GMl-enabled KG engine. 
Section~\ref{sec:arch} presents the {\sysName} platform. 
Section~\ref{sec:eval} discusses the results of evaluating our automated pipeline for training GML models.
Sections~\ref{sec:related_work} and ~\ref{sec:conc} are related work and conclusion.

% In Section \ref{sec:related_work}, we review the related work. Section~\ref{sec:conc} concludes.






==> sections/introduction-old.tex <==
\section{Introduction}
\label{sec:intro} 

\begin{figure}[t]
\small
\centering
  \includegraphics[width=0.85\columnwidth]{figures/Paper_Venue_KG_DBLP.pdf}  % \ncp\ncp\ncp\ncp\ncp
  \caption{A KG with nodes/edges in red, which could be predicted by classification and link prediction models on the fly.\shorten}
  \label{fig:Paper_Venue_KG}
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp
\end{figure}

\begin{figure}[t]
\lstdefinestyle{myStyle}{basicstyle=\small\ttfamily, language=SPARQL, alsoletter{:} }
\begin{lstlisting}[style=myStyle,captionpos=b,showspaces=false,frame=singlem,numbers=left,xleftmargin=0.5cm,morekeywords={kgnet, getNodeClass,dblp},escapechar=\%]
prefix dblp: <https://www.dblp.org/>
prefix kgnet: <https://www.kgnet.com/>
select ?title ?venue
where { 
?paper a dblp:Publication.
?paper dblp:title ?title.
?paper %\textbf{?NodeClassifier}% ?venue.
?NodeClassifier a %\textcolor{purple}{ \textbf{kgnet:NodeClassifier}}%.
?NodeClassifier kgnet:classifierTarget dblp:paper.
?NodeClassifier kgnet:classifierLabel dblp:venue.}
\end{lstlisting}
\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{A SPARQL GML-enabled query that use a node classification model to predict a paper's venue on the fly.}
\label{fig:paperVenueSPARQL}
\ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\end{figure}

A knowledge graph (KG) integrates heterogeneous datasets from diverse data sources based on semantics~\cite{Knowledge_Graphs_Hogan}. Graph ML techniques, such as graph representation learning, link prediction, graph matching, and node classification, play an essential role in graph machine learning and graph semantics understanding.  
%
Extending KG engines with these techniques will lead to a new class of queries that use representation learning and graph machine learning (GML) models to search and explore a KG based on semantics. We refer to this new class as \textit{GML-enabled Query}, which will enrich data discovery and generate hidden insights. Existing KG engines lack support for GML-enabled queries. basically, these engines support logical, arithmetical, and rule-based inference  operators in the query. In relational databases, ML-enabled (Cognitive) queries were introduced by \cite{bordawekar2017cognitive} and focused on learning representations for database tokens, i.e., words. 

For KGs, enabling ML-based queries is a more challenging task due to the dynamic schema of KGs and a wide range of KG embedding (KGE) and graph neural network (GNN) methods that could be used in several applications for heterogeneous graphs \cite{GNN_Survey_2021,KG-link-prediction,KG-Embedding-Survey}.
%
The KG schema illustrated in Figure~\ref{fig:Paper_Venue_KG} contains information about published papers in DBLP~\cite{KG_DBLP} that are stored in RDF format for RDF engines. Traditional SPARQL query language cannot apply ML tasks on top of KG data i.e. predict a class for graph node, predict a missing link between two nodes, or predict a class for a sub-graph of nodes. These ML applications are widely studied recently by GNN methods \cite{GNN_Survey_2021}. 

The venue node in the schema is a virtual node that does not exist in the KG so \textbf{is it possible to get the paper-venue  node using a GML node classifier by writing a SPARQL query?} Writing GML-enabled query \emph{(GML-Q)} for the previous task is applicable. we need to link between SPARQL language and GML node classification methods that are able to learn a class for each  target node based on graph structure and target node-associated features. These methods essentially generate an embedding for each target node and feed it to a Sigmoid layer for classification \cite{GCN}.
Figure \ref{fig:paperVenueSPARQL} shows a GML-Q that extends a SPARQL query to predict a venue for each paper using the system-defined GML-Operator \textbf{\emph{kgnet:NodeClassifier}}. 

The GNN trained \emph{"NodeClassifer"} takes the paper node as input and returns the venue as output. The returned labeled nodes are formulated as RDF triples that will be added to the KG. The classifier and all of its associated properties/parameters are stored inside a trained models registry that is represented under the graph prefix \textbf{kgnet} as RDF triples that can be queried and customized for data science tasks. 

the GML-Operator makes a call to a GNN-trained classifier that samples the set of relations and nodes surrounding each target node,i.e. the authors of the paper, the affiliation of each author, the year of publication, and the citation links between papers, that are logically sufficient to define to which venue this paper could be published-in then learn and infer the venue (class). similarly, link prediction and other applications can be applied.

There are many techniques to generate representations (embeddings) that capture the semantics of graph data. For examples, geometric-translational methods such as (TransE, CrossE, and RotatE) in ~\cite{KG-Embedding-Survey}, non-linear semantic methods such as (HolE, ComplEx, and DistMult) in \cite{KG-link-prediction}, deep learning methods such as (ConvE, ConvR, and RSN) in \cite{KG_LP_Survey}, and GNN methods such as (RGCN, Graph-SAINT, and GAT) in \cite{GNN_Survey_2021}.Many semantic similarity scoring metrics exist, such as Euclidean distance, Cosine, and Jaccard, to measure the semantic similarity based on the distance between two embeddings \cite{Semantic-Similarity-Survey}.  
% Thus, it is time-consuming and challenging to build AI pipelines that extract semantic information from KGs using GML methods as it requires a deep understanding of these methods and variations of their implementations. 

In this paper, we propose {\sysName}, a knowledge graph machine-learning enabled RDF engine. {\sysName} extends existing RDF engines with a \textit{GML-enabled query operators} that interacts with an embedding store and GML services, where we support a repository of GNN methods, KGE methods, and similarity measure metrics. {\sysName} \textit{Interface} provides GML task creator to help the user writing a GML-enabled query and get results. 

{\sysName} extend a SPARQL query engine with GML operators to train and use GML models where model metadata are stored in the KG for later data science operations. Users can query and update trained model metadata using SPARQL queries. The GML-enabled query engine addresses several research challenges,  such as 1) deciding the GML method that best fits the user  query i.e. the task required resources for a given KG such as the task type (GML operator), the available compute resources, and the user budget (preferences). 2) estimating the cost of executing GML operators. 3) optimizing cognitive query through query re-rewriting and execution pipeline. and finally, 4) a KG data sampler that samples a smaller sub-graph that is related to the task to avoid full graph training for higher performance and scalability. A basic node similarity search implementation of {\sysName} is demonstrated in \cite{KGNET_DEMO}.

{\sysName} is a proof-of-concept system that poses several research opportunities for developing a scalable GML-enabled KG engine. We evaluated {\sysName} using three graph ML tasks on real KG datasets that require different GML methods. 
% The use cases cover applications, such as economics, question-answering, and security.  
{\sysName} enables a user to run a GML task using a SPARQL-Query without a prior experience in machine learning for KG.

The remainder of this paper is organized as follows. Section~\ref{sec:ChallengesOfAutomatingCognitiveQuery} outlines the main research challenges of developing  a GMl-enabled KG engine. Section~\ref{sec:arch} presents an architectural overview of {\sysName}. Section~\ref{Use-cases} evaluates {\sysName} using three uses cases. In Section \ref{sec:related_work}, we review the related work. Section~\ref{sec:conc} concludes.





==> sections/pipeline.tex <==
\section{{\sysName} and GML Automation on KGs}
\label{sec:kg-tosa} 
In this section, we introduce the {\sysName} end-to-end pipeline steps to apply GML tasks on top of KGs using GNNs. Training GML task on top of KG as illustrated in figure \ref{fig:KG-TOSA_Pipeline} takes the KG, GML task, task budget constraints, and available computing resources as input then produce the task results in a JSON format as an output. The pipeline has multiple integrated components (steps). The first component is a SPARQL-based sub-graph extractor that extracts the KG triple in a CSV raw format and feeds it to the second component, the data set transformer, that transforms the raw triples into adjacency matrix format and applies dataset train-valid-test splitting. The third component, GNN method selector, starts to optimize for the best GNN method that fits the task budget and available resources. The graph machine learning component (GML) starts to load the transformed dataset into memory, sample-train-validate the dataset, and save the trained model into a model file. Finally, the KG-GNN inference component loads the saved model and produces the output into a JSON format through a Restful API response. This pipeline has a modular design that enables adding multiple GNN methods, sampling methods, and optimization rules. The details of these components are explained as follows.

\begin{figure}[t]
  \centering
  % \includegraphics[width=250]{figures/TOSA Architecture.pdf}
  \includegraphics[width=\columnwidth]{figures/GMLPipeline.pdf}
  \caption{{\sysName} GML pipeline. }
  \label{fig:KG-TOSA_Pipeline}
  \ncp\ncp\ncp\ncp\ncp
\end{figure}



\nsstitle{\textbf{KG-Sampler.}}
To prepare a heterogeneous graph dataset for GNN training, existing research considers manually preparing the dataset from various sources in a proper format for their training framework. Heterogeneous graphs are by definition a form of KGs. There are multiple knowledge graphs engines exist that enable CURD operation on KG data i.e. Open-link Virtuoso \cite{Virtuoso}, Apache Jena, Star-dog, and others. To avoid moving the full KG data outside the engine to extract the proper dataset, {\sysName} uses Open-link virtuoso to load the KG data and then uses SPARQL language to extract the proper dataset. Using SPARQL we can define various BGPs to extract a sub-graph with a specific pattern. The BGP can be a manually designed query or one of the BGP catalog queries supported by the system for auto-selection. As {\sysName} is focusing on task-oriented sampling, the system currently supports 4 different one-batch sampling BGPs namely (SQ, BSQ, PQ, and BPQ) as shown in figure \ref{fig:GNN_subgraph_sampling}.c.

\nsstitle{\textbf{Dataset Transformer.}}
In order to train GNN methods on a KG triples dataset, the triples are extracted from KG using a BGP SPARQL query into a raw TSV/CSV format. Then, all triples are converted into an adjacency matrix format that represents the graph structure in memory. This format is compatible with Py-Geometric \cite{pytorch-geometric-Dataloader} and DGL\cite{DistDGL} the most common graph ML data loaders. These graph loaders are optimized for sparse heterogeneous graphs i.e., knowledge graphs \cite{KG-Sparsity}. The data loader loads the adjacency matrix and converts it into a memory sparse matrix representation. This representation is optimized for memory allocations and sparse-matrix operations. 

Data prepossessing steps start to check the consistency of graph data by validating node/edge types counts, applying custom user filters needed, removing the target class edges if it is there, and generating statistics about the graph (nodes, edges, and relations). Then, the data encoding step starts to encode each node and edge type into a unique id. The nodes mapping step creates a separate CSV file for each node type that maps between the original graph node URI and the given id besides converting literal values into nodes. The adjacency matrix mapping step creates a separate CSV file for each edge type (relationship) by replacing the original node URIs with their given ids. Data splitting step split target nodes into train-validation-test splits according to different strategies i.e., (Random splitting: using sklearn-learn random train-test split, Community-based: using one of the edge types that is able to provide a logical data splitting semantic for the task). 
Finally, the generated dataset-files structure is zipped into one file that is used as the input dataset for the GNN method trainer. {\sysName} is the first to automate this transformation to enable ad-hoc task-oriented GML tasks.

\nsstitle{GNN Method Selector.}
As {\sysName} supports a catalog of KG-GNN methods that have different efficiency and scalability levels, the system can optimize for the GNN method that best fit the given GML task and task budget. All of these methods share the Relational Graph Convolutional Networks (RGCN) as the core layer inside their model's implementation. The sampling methods cost basically depends on the sampling heuristic and the definition of neighbor nodes which can be up to 50\% of the training time in many methods \cite{Serafini21}. {\sysName} optimizer can decide the resources required for each method and optimize for the best-fit method based on the task budget constraints and the available resources. This selection  enables better scalability in a distrusted environment settings as a future direction.

\nsstitle{GML Training.}
The GNN training process starts with loading the Adjacency metrics dataset for the selected GNN method using one of the graph sparse tensor loaders, e.g., PyG and DGL. {\sysName} use these loaders as they are the most common loaders used with large graph datasets as both support optimized sparse tensors for optimized memory and optimized sparse matrix operations. Moreover, these libraries support CPU/GPU modes in training besides a distributed training setting for many methods \cite{DistDGL}. After dataset loading, the GNN method starts the training and validating steps. Meanwhile, the sampling steps are interleaving for GNN sampling-based methods. After training is complete the evaluation metric is reported and the trained model is saved into a model file for later inferencing tasks.

\nsstitle{\textbf{GML Inferencing.}}
{\sysName} inferencing is the output component that is responsible to answer the original GML task. The saved model is loaded again into memory and the GNN inference function can infer a class for each node in the node classification task or the top-k links in the link prediction task. The output is serialized into a JSON Restful-API response for easy and lite integration with other front-end services.


==> sections/usecase_old.tex <==
\section{{\CKGS} in Practice}   
\label{Use-cases}

Several use-cases that cognitive intelligence queries~\cite{bordawekar2016enabling} can help to solve are already found especially in the era of big data and heterogeneous distributed graphs databases. For Example, in the computer vision domain, measure similarity between two persons using their photos features is now available, you can combine such semantic search ability with structured person data that can help to improve surveillance systems validity~\cite{zafar2019face}.In another domain, Drug-drug interaction embedding does not only reduce the number of interference cases but can also result in a reduction of drug development\cite{drug-drug-interaction}. Question answering is another use case that can benefit from cognitive queries that help natural language processing systems to extract similar search keywords using a word embedding techniques \cite{Wan_QA2020}. In this section, we show three different use-cases to demonstrate how SPARQL engines can benefit from such joint embedding integration.


\subsection{Question-Answering on KGs}
QA use-case highlights the power that cognitive SPARQL queries can provide to question answering NLP problems. Assume you have a question answering system that allows the user to query over a DBpedia graph using natural English language phrases. QA system will firstly pre-process the given phrase trying to extract keywords from that phrase. then try to construct a SPARQL query to search for entities and relations that are related to the keywords list. In that case, if there isn't a relation or entity that matches the given keywords list the SPARQL query result will be empty. Imagine you are able to fetch another list of semantically related words to the given keywords list and able to sort them according to the level of similarity. Finally, you end up with a SPARQL query that can answer your question in a cognitive way just by add semantic similarity UDF \textbf{getGloveSimilarity} to your query. the following is a sample of SPARQL query that query DBpedia dataset (loaded into Virtuoso server from Turtle files dump) including joint embedding that searches for similar words based on pre-trained Glove \cite{glove} model. Figure \ref{figure:takeplace} shows example of a SPARQL query and table \ref{tbl_QueryTakePlaceResult} show results.
\begin{figure}[h!]
  \centering
  \begin{tcolorbox}[colback=red!1!white,colframe=black,
    title=SPARQL Query: select similar words to "take place"]
    select distinct  ?p, STRAFTER(str(?p),'/property/') 
    As ?label,
    (\textbf{sql:getGloveSimilarity}(STRAFTER(str(?p),
    '/property/'),'take place')) AS ?Score
    where \newline
    \{
    \newline
    <http://dbpedia.org/resource/Boston\_Tea\_Party> ?p ?o.
    \newline
    filter(strlen(STRAFTER(str(?p),'/property/'))>0)
    \newline
    \}  
    \newline
    ORDER BY 
    \newline
    DESC(sql:getGloveSimilarity
    (STRAFTER(str(?p),'/property/'),'take place'))
    LIMIT 300
    \end{tcolorbox}
  \caption{A SPARQL query selects similar predicates to "take place".
  \label{figure:takeplace}}
\end{figure}
\input{tables/table1}


\subsection{Semantic Linking for Heterogeneous Data}
President face similarity use-case highlights the power that cognitive SPARQL queries can provide to KG that jointly linked with image dataset like \textbf{Wikidata} and \textbf{WikiMedia}. In this use-case we tried to build KG linked with images. we used Wikidata to build a dataset contains countries and their current president information like (name, sex, date of birth, photo (URL from Wikimedia), and list of previous positions). Then built an RDF graph from that dataset where presidents URI represent the subject, information feature represent predicate followed by information literal value as an object. Graph serialized as Turtle file and loaded to Virtuoso server. 
\newline
\newline
OpenCV MCTNN \cite{MTCNN} had used To extract faces from photos followed by a pre-trained FaceNet\cite{facenet} model that produces a vector of 512 dimensions that represent embedding for each face. Faces embedding loaded in memory at a web service and can be queried using UDF called \textbf{getFaceNetSimilarity} that return similarity score between two presidents URIs. Also, you can use an external image URL to get a list of presidents who are similar to the external photo. Figure \ref{figure:JoeBiden} show a Cognitive SPARQL query that uses joint Face embedding to filter query results. this query asks for presidents who looks-like USA president "Joe Biden" and results are shown in table \ref{tbl_QueryJoeBidenResult}.
\begin{figure}[h!]
  \centering
  \begin{tcolorbox}[colback=red!1!white,colframe=black,
    title=SPARQL Query: select president who looks-like "Joe Biden"]
    prefix wd:<http://www.wikidata.org/entity/>
    \newline
    prefix ns1:<http://www.wikidata.org/property/>
    \newline
    select * where
    \newline
    \{
    \newline
    ?s ns1:name ?o. 
    \newline
    \{
    \newline
        select ?o,((\textbf{sql:getFaceNetSimilarity}('joe biden',?o)) As ?Score)
        where 
        \newline
        \{
        \newline
            ?s ns1:name ?o. 
            \newline
        \}
        \newline
    \}
    \newline
    \}
    order by DESC(?sim)
    \end{tcolorbox}
  \caption{SPARQL query that select president who looks-like "Joe Biden".\label{figure:JoeBiden}}
\end{figure}
\input{tables/table2}
User can also use an external image (i.e The American singer James Buffett) to measure similarity as shown in Query \ref{figure:JamesWilliamBuffett} and table \ref{tbl_QueryJamesWilliamBuffettResult}.
\begin{figure}[h!]
  \centering
  \begin{tcolorbox}[colback=red!1!white,colframe=black,
    title=SPARQL Query: "James Buffett" looks-like query]
    prefix wd:<http://www.wikidata.org/entity/>
    \newline
    prefix ns1:<http://www.wikidata.org/property/>
    \newline
    select * where
    \newline
    \{
    \newline
        ?s ns1:name ?o. 
        \newline
    \{
    \newline
        select ?o,((\textbf{sql:getFaceNetSimilarity}('https://www.
        \newline
        grunge.com/img/gallery/the-untold-truth-of-jimmy-buffett/intro-1579893853.webp',?o))
        \newline As ?sim)  where 
        \newline
        \{
        \newline
            ?s ns1:name ?o. 
            \newline
        \}
        \newline
    \}
    \newline
    \}
    order by DESC(?sim)
    \end{tcolorbox}
  \caption{SPARQL Query: select president who looks-like Singer "James Buffett" using External URL.\label{figure:JamesWilliamBuffett}}
\end{figure}

\input{tables/table3}


We have to note that, using external images with SPARQL engine takes more time to generate results because every time the UDF requests the web service to calculate similarity it has to extract face and generate embedding then calculate Cosine similarity score with each candidate. To solve this issue we used a simple cashing mechanism that cash each external URLs with their embedding vector in memory to fetch it faster in the next requests. Although this works with small datasets it has to be investigated more for large datasets.


\subsection{Semantic Classification and KG Embeddings}


==> tables/table1.tex <==
\begin{table*}[ht]
\ncp\ncp
 \centering
 \small
  \caption{Use cases baaed on real datasets, various embedding/classification techniques, and KG augmentation.}
  \ncp\ncp\ncp\ncp\ncp\ncp
  \label{tbl_usecases}
  \begin{tabular}{|p{14em}|p{11em}|p{12em}|p{9em}|p{9em}|}
    \hline
    \hfil \textbf{}& \hfil \textbf{KG With Images}&  \hfil \textbf{Economics}&  \hfil \textbf{QA} &\hfil \textbf{Data Security}\\
    \hline
    \textbf{Dataset}&Dog Breeds&Forbes-2018&DBPedia-2016-10&DoHBrw-2020\\
    \hline
    \textbf{Data Source} &  \href{https://www.kaggle.com/harisalikhan/dog-breeds}{\color{blue}{Kaggel}} + \href{https://data.world/nicolemark/dog-breeds-dataset-enrichments/workspace/file?filename=dog+breeds_enriched_20210503.csv}{\color{blue}{Data.World}} & \href{https://data.world/aurielle/forbes-global-2000-2018}{\color{blue}{Data.World}}& \href{https://downloads.dbpedia.org/wiki-archive/downloads-2016-10.html}{\color{blue}{DBPedia}}&\href{https://www.unb.ca/cic/datasets/dohbrw-2020.html}{\color{blue}{CIRA-CIC}}\\
\hline
 \textbf{\# Entities}& 132 dog breeds& 2000 companies & NA&4000 incident\\
 \hline
  \textbf{Embed. Models}& VGG16 &
RDF2Vec ,TransE, .. &GloVe&RDF2Vec ,TransE, .. 
 \\
\hline
 \textbf{Embedding Generation}& On fly & While graph loading & On fly & While graph loading \\
\hline
 \textbf{UDF}& getDogSimilarityScore & getSimilarCompanies & getSimilarKeywords& getSimilarAttacks \\
\hline
 \textbf{Embed. Type}& Image Embedding& KG Embedding&
KG Embedding&KG Embedding\\
\hline

 \textbf{Classification Model}& VGG16& Random Forest& NA&Random Forest\\
 \hline
 \textbf{KG Augmentation Technique}&Linking with other datasets & Attribute Classification  &NA&NA\\
\hline
\textbf{KG Augmented With} & \href{https://bowwowinsurance.com.au/dogs/dog-breeds/akita/}{\color{blue}{bowwowinsurance.com}} &3 Quantiles Values (L,M,H) &NA&NA\\
\hline
 \textbf{{\sysName} Query time\//sec} & 36.5& 2.4& 3& 5.03 \\\hline
 \textbf{Python Script time} & 29.5s +25m train time & 0.51s +1.6m train time &2.7s+30m train time &2.3s+1.8m train time \\\hline
 \textbf{\# {\sysName} Query code lines} & 21 & 20 & 19& 13 \\\hline
 \textbf{\# Python Script code lines} & 240 & 197 & 133 & 179 \\\hline
\end{tabular}
\ncp\ncp\ncp\ncp\ncp\ncp
\end{table*}

==> tables/table1_GNN_v0.tex <==
\begin{table*}[ht]
 \centering
 \small
   \caption{The {\sysName}'s training pipeline is evaluated using two real KGs. Due to our task-oriented sampling, we managed to use four times larger KGs (DBLP and Yago) than the ones reported in OGB~\cite{OGB}. We used GML methods, such as RGCN~\cite{RGCN}, GraphSAINT~\cite{GraphSAINT}, and ShadowSAINT~\cite{Shadow-GNN} for Node Classification (NC) tasks, MorsE~\cite{MorsE} for Link Prediction (LP) tasks, and GraphSIANT\cite{GraphSAINT} for Similar Entity (SE) tasks.}
  \label{tbl_GNN_usecases}
  \begin{tabular}{|p{8em}|p{4em}|p{17em}|p{6em}|p{6em}|p{4em}|}
    \hline
    \hfil \textbf{Knowledge Graph}&  \hfil \textbf{\#Triples} &\hfil \textbf{\#Targets}&\hfil \textbf{\#Edge Types}&\hfil \textbf{\#Node Types}&\hfil \textbf{Tasks}\\
    \hline
    % \href{https://ogb.stanford.edu/docs/nodeprop/#ogbn-mag}{\color{blue}{OGBN-MAG}} \cite{OGB}&62M&349 Venue&4&4&NC\\
    % \hline
 \href{https://blog.dblp.org/2022/03/02/dblp-in-rdf/}{\color{blue}{DBLP}}&252M&50 Venue,51283 Affiliations,1.2M paper&62&22& NC,LP,ES\\
    \hline
    \href{https://yago-knowledge.org/downloads/yago-4/}{\color{blue}{YAGO4}}&250M&50 Country&156&73& NC \\ \hline
\end{tabular}
\end{table*}

==> tables/table2.tex <==
\begin{table}
  \caption{SPARQL "Joe Biden looks-like" query result.}
  \label{tbl_QueryJoeBidenResult}
  \begin{tabular}{ccl}
    \toprule
    s&o&Score\\
    \midrule
http://wikidata.org/entity/Q6279 & Joe Biden & 1\\
http://wikidata.org/entity/Q94941 & Fred VII& 0.87\\
http://wikidata.org/entity/Q57392 & Armando Gu & 0.83\\
http://wikidata.org/entity/Q156572 & Christ VII& 0.75\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/table3.tex <==
\begin{table}
  \caption{SPARQL "James Buffett" looks-like query result.}
  \label{tbl_QueryJamesWilliamBuffettResult}
  \begin{tabular}{ccl}
    \toprule
    s&o&Score\\
    \midrule
http://wikidata.org/entity/Q295141&Chaim H&0.40\\
http://wikidata.org/entity/Q8573&Sun Yat-sen&0.37\\
http://wikidata.org/entity/Q152369&Fouad M&0.34\\
  \bottomrule
\end{tabular}
\end{table}
